A Note on Latency Variability of Deep Neural Networks for Mobile Inference

Running deep neural network (DNN) inference on mobile devices, i.e., mobile inference, has become a growing trend, making inference less dependent on network connections and keeping private data locally. The prior studies on optimizing DNNs for mobile inference typically focus on the metric of average inference latency, thus implicitly assuming that mobile inference exhibits little latency variability. In this note, we conduct a preliminary measurement study on the latency variability of DNNs for mobile inference. We show that the inference latency variability can become quite significant in the presence of CPU resource contention. More interestingly, unlike the common belief that the relative performance superiority of DNNs on one device can carry over to another device and/or another level of resource contention, we highlight that a DNN model with a better latency performance than another model can become outperformed by the other model when resource contention be more severe or running on another device. Thus, when optimizing DNN models for mobile inference, only measuring the average latency may not be adequate; instead, latency variability under various conditions should be accounted for, including but not limited to different devices and different levels of CPU resource contention considered in this note.

==> algorithm.tex <==
%\subsection{\Capname Capacity}

\section{\ouralg: Tenant Sprinting Through \Capname Capacity}


In this section, we discuss whether it is feasible to exploit
under-utilized \capname capacity in practice, and then present \ouralg
to utilize \capname capacity for tenants' sprinting in \multis.

%present \ouralg to exploit the under-utilized \capname
%capacity. We first

\subsection{Feasibility of Utilizing \Capname Capacity}\label{sec:existence_of_unused_capacity}

%
%
%\textbf{Implications of capacity overloading.}
As illustrated in Fig.~\ref{fig:datacenter_diagram},
data centers impose capacity constraints at different hierarchies for safety.
The operator manages
the capacity at data center and PDU levels serving multiple tenants, while individual tenants
control their power usage below contract capacity at the rack level. Capacity overloading can occur
at all these levels, but have very different implications.


\emph{Data center level.} When overloaded, UPS will enter the ``bypass''
mode and utility power will directly feed into PDUs without UPS protection.
Further, as cooling capacity is sized based on the IT critical
power, overloading UPS also means overloading the cooling capacity,
which significantly increases outage risks.\footnote{Recent research \cite{JasonMars_Thermal_Time_Shifting_ISCA_2015_Skach:2015:TTS:2749469.2749474} has proposed to place phase changing materials directly into servers to mitigate cooling loads, but tenants' servers may not have such advanced materials.} In addition,
overloading capacity at the data center level may entail
a heavy penalty on the operator due
to its violation of power demand contract with utilities \cite{Fan:2007:PPW:1250662.1250665}.
Thus, overloading at the data center
level is extremely undesirable.

\emph{PDU level.}
%Since each PDU is often served by one air handler unit (an indoor cooling
%unit used in conjunction with chillers)
Since one air handler unit is typically sized
to maintain the designed power density across the racks served by the PDU,
a risky consequence of PDU-level overloading is that
the average server heat density exceeds the air handler's capacity and results
in overheating. Additionally, the circuit
breaker at the PDU may trip in the event of overloading. Thus,
it is also very risky to overload the PDU-level capacity.

\emph{Rack level.} While rack-level capacity is enforced through
a circuit breaker, tenants' rack-level power usage is primarily
limited due to \emph{contract} reasons rather than infrastructure constraints.
For example, using a cross-connected and shuffled
power delivery architecture \cite{Umich_PowerRouting_ASPLOS_2010_Pelley:2010:PRD:1736020.1736047},
unused capacity at the PDU level can be dynamically delivered
to overloaded racks without tripping the rack-level circuit breaker (called
power routing).
Moreover, the rack-level circuit breaker capacity (approximately US\$1 per watt) is a negligible
fraction of the total infrastructure cost \cite{Umich_PowerRouting_ASPLOS_2010_Pelley:2010:PRD:1736020.1736047}.
Hence, over-sizing the rack-level capacity
while limiting its actual allowed usage
through software control (called
soft ``fuses''
 \cite{PSU_StatisticalProfiling_EuroSys_Govindan09}) can
 better utilize the more expensive capacities at UPS and PDU
 levels. Last but not least, even without power
routing or soft ``fuses'', tenants' contract capacity
can still be exceeded by 25\% temporarily (for, e.g., handling occasional load spikes) with negligible increased downtime risks, since it
is currently limited at 75-80\% of the circuit
breaker's rated capacity. On the other hand,
the circuit breaker is designed to sustain
 loads at 100\% utilization for at least three hours continuously, not to mention the circuit breaker's
tolerance itself (e.g., it can
take two hours to trip a rack-level circuit breaker
at 120\% of its rated capacity \cite{Xiaorui_ICAC_2011_Power_Oversubscription_Fu:2011:MPO:1998582.1998589}).
Note further that one tenant's exceeding its rack-level contract capacity by 25\% will not cause
overheating problems, as long as the air handler capacity (decided
based on PDU capacity)
is not violated.

In sum, overloading the data center-level UPS or PDU
capacities is very dangerous, while over-provisioning
their capacity during construction is expensive and
 increasing capacity
at runtime is practically impossible.
The rack-level capacity, however, can
be over-provisioned with little extra cost
and/or dynamically supplied based on actual needs
(via power routing \cite{Umich_PowerRouting_ASPLOS_2010_Pelley:2010:PRD:1736020.1736047} or soft fuses \cite{PSU_StatisticalProfiling_EuroSys_Govindan09}).
Therefore, even when a tenant reaches or even marginally exceeds its rack-level contract capacity,
there is no danger at all, because
there is still unused capacity at the rack-level circuit breaker (either
intentionally over-provisioned \cite{PSU_StatisticalProfiling_EuroSys_Govindan09} or dynamically delivered \cite{Umich_PowerRouting_ASPLOS_2010_Pelley:2010:PRD:1736020.1736047}).
Nonetheless, the  static
contract capacity unnecessarily limits tenants' power usage at rack levels,
creating an \emph{artificial} hurdle that prevents
utilization of  \capname capacity for tenants' sprinting.




\subsection{Managing \Capname Capacity}


While tenants need \capname capacity for sprinting
during peak loads
and it is safe to let tenants exceed their rack-level contract capacity,
a careful scheme to manage the \capname capacity must be in place.
%Further, we must avoid
%tenants' abuse of \capname capacity (e.g.,
%using it as their normal contract capacity) while
%offering it as a discounted resource.
%To study the economic feasibility,
Here, for case study, we consider a variant of token-based
\capname capacity management which includes the following
rules.



$\bullet$ \emph{Reservation capacity.}
On top of the normal contract capacity that
can be continuously utilized up to 100\%, each participating tenant can make
a reservation on  \capname
capacity at a discounted price, which
sets a limit on the maximum \capname capacity that a tenant
can utilize. In other words,
 the maximum rate at which a tenant can spend its token is
 limited. Each token represents one kWh (one kW for one hour).

$\bullet$  \emph{Token purchase.} Tenants need to purchase tokens
from the operator at specified prices. They
can only buy tokens when their power demand is
below the contract capacity, and
the maximum rate at which tenants can get tokens
is proportional to the difference between their
contract capacity and actual power demand (i.e.,
the lower power demand, the faster token accumulation).



$\bullet$ \emph{Limits.} Tenants spend tokens when their power demand
exceed contract capacity subject to the limit
on their spending rates. If a tenant violates
its spending rate and/or overdraws its tokens, it may face power cut, incur additional
penalties, and/or be disallowed
to use \capname capacity in the future.
To prevent tenants from
 using \capname capacity at 100\% utilization for a prolonged
 period of time,
we also set a limit on the amount of tokens that tenants can accumulate
over time. %Tokens beyond the limit are removed from tenants' account.
Note that we do not impose constraints on \emph{when} sprinting
is allowed provided that tenants have tokens.
While this may increase tenants' aggregate peak demand
and require the operator to provision extra capacity to accommodate
sprinting, our case study in Section~\ref{sec:simulation} shows that the operator
can still make extra profit.
In our future work, we will study more advanced mechanisms
(e.g., dynamic pricing) that further
restricts when tenants' sprinting can occur.

%In sum,
%we use  a simple token-based mechanism
%to investigate the economic benefits
%of allowing tenants' sprinting.
%

























==> model.tex <==
\section{Model}
There are $N$ tenants with power subscription of $P_i^o$ for $i=\{1,2,\cdots ,N\}$. Each tenant have a virtual battery with peak discharging rate capacity $P_{i,discharge}$, peak charging rate $P_{i,charge}$, and maximum energy capacity $E_{i,max}^{b}$.For convenience we choose to represent charging as +ve power for battery. Tenant $i$'s instantaneous power consumption is $P_i(t)$. Now when $P_i(t)>P_i^o$ tenants discharge battery to offset the subscription violation. On the other hand, when tenants' power is less than the subscribed capacity it can charge its battery if the battery energy level is less than its capacity. The charging and discharging rate for any decision time slot depends on battery's current energy level. Denoting the tenants battery power as $P_i^{b}(t)$ and energy level as $E_i^{b}(t)\leq E_{i,max}^{b}$ we can write
\begin{eqnarray}
P_i^{b}(t)=\begin{cases}
P_i^o-P_i(t)\geq  \max\{-\frac{E_i^{b}(t)}{t},P_{i,discharge}\}, \text{when } P_i(t)>P_i^o \\
\min\{\frac{E_{i,max}^{b}- E_i^{b}(t)}{t},P_{i,charge}\}, \text{otherwise} 
\end{cases}
\end{eqnarray}
where $t$ is the time slot length. Note that as tenants discharge capacity or offset capacity depends on its current battery level, therefore it must employ additional power capping method when there is not enough battery capacity left.

The energy level of battery evolve as follows
\begin{eqnarray}
E_i^b(t+1) = \left[E_i^b(t)+t\cdot P_i^{b}(t)\right]_0^{E_{i,max}^{b}}
\end{eqnarray}

The battery power for operator $P_o^b(t)$ can be expressed as follows
\begin{eqnarray}
P_0^b(t) = \min\{\sum_{i=1}^{N}\left[P_i^0-P_i(t)-P_i^{b}(t)\right],\frac{E_{0,max}^b(t)-E_0^b(t)}{t}\}
\end{eqnarray}

The energy level of operator's battery evolve as follows
\begin{eqnarray}
E_0^b(t+1) = \left[E_0^b(t)+t\cdot P_0^{b}(t)\right]_0^{E_{0,max}^{b}}
\end{eqnarray}

==> simulation.tex <==
\section{Case Study}\label{sec:simulation}


%We conduct a case study of using power-trade in a multi tenants data center, and study the potential benefits for tenants and operator. We also study how different scenarios and pricing affects their benefits.

We now present a case study to
highlight benefits of exploiting \capname capacity,
which helps data center operator receive extra
profits and meanwhile makes capacity {sprinting}
a reality for tenants to avoid performance degradation in \multis.
More concretely, our study shows that data center operator
can increase its profit by up to 35\% (compared
to the case without utilizing \capname capacity), while
tenants can save more than 15\% without
performance losses (compared to leasing capacity
at full prices).

%\textbf{\color{red}I stopped here.}

\subsection{Methodology}


We perform a simulation study based on power traces
collected from multiple racks in a \multi. As the tenants' capacity leasing information
is not available for privacy reasons,
we scale the power data and consider that they belong
to five different tenants, which all have the same contract
capacity and share one PDU/air handler.
In our study, we determine capacity oversubscription levels based on emergency/overloading probability,
e.g.,  3\% emergency for the operator means
it maximally oversubscribes the PDU capacity while ensuring that the emergency probability
is no more than 3\%.\footnote{PDU/UPS overloading is the operator's
fault that is dealt as an orthogonal
issue (e.g., \cite{Shaolei_Colocation_Power_Capping_HPCA_2016}) beyond the scope of this paper.}
Note that tenants' emergency refers to the event of
\emph{contract} capacity overloading and that
depending on
both tenants' and operator's oversubscription levels under evaluation,
each tenant's contract capacity will vary.
By default, the operator provisions its capacity exactly based on tenants'
aggregate demand with zero emergencies. Thus, when
tenants' sprinting is allowed, the operator needs
to provision more capacity. This is because our simple
token-based mechanism does not restrict when tenants
can spend tokens for sprinting, which
may increase tenants' aggregate demand.
Such extra capacity investment is also factored into our cost analysis.



The operator
offers a contract capacity leasing rate of US\$150/kW/month (without
additional energy charge), and
its infrastructure capacity cost is set as US\$15/W with a 15-year life cycle,
which is amortized as approximately US\$84/kW/month.
We consider an average electricity price of 10\textcent/kWh,
and the data center has
a power usage effectiveness of 1.5.
For \capname capacity,
the \emph{default} reservation price
is set to 30\$/KW/month (i.e., only 20\% of the normal contract
capacity charge), and the usage charge (i.e., price for purchasing
tokens) is
 20\textcent/kWh, which is the tenant's equivalent energy
 price obtained by dividing the contract capacity price of US\$150/kW/month by the maximum
energy usage of 720kWh/month under 100\% utilization.
We will vary these values in our experiments.
%We study the impact of different reservation and usage charge on operator and tenants' benefit.
To focus on \capname capacity,
 we exclude from our study those
 costs (such as administrative and space) that are not relevant to power/cooling capacity.



In our evaluation, we consider
the following
metrics.

$\bullet$ \emph{Operator's profit increase.}
We calculate the operator's profit increase due to \ouralg, compared
to the baseline case without using \ouralg. The profit
is calculated as the difference from the operator's
revenue (of leasing capacity to tenants,
including \capname capacity if applicable)
and its cost (both amortized infrastructure cost and
energy cost).

$\bullet$ \emph{Tenants' cost saving.} We show
 tenants' cost reduction by exploiting \capname capacity
for capacity sprinting that avoids
performance losses, compared to the case where tenants
have to lease the capacity at the full price of US\$150/kW/month.
Tenant's cost includes contract capacity charge and reservation/usage
charges for \capname capacity (if applicable).


In addition, we also run experiments to show the performance improvement
that \ouralg brings to tenants compared to the case where tenants
cap their power demand under the contract capacity.


\subsection{Evaluation Results}


Next, we show our evaluation results and demonstrate
the mutual benefits of \ouralg under different settings.


\subsubsection{Economic Benefits}


\begin{figure}[!t]
	\centering
	\subfigure[]{\label{fig:opSave_impact_reserv_charge}\includegraphics[trim=2cm 9cm 1cm 9cm,  clip, width=0.23\textwidth,clip]{../figures/opSave_impact_reserv_charge2}}
	\subfigure[]{\label{fig:tenSave_impact_reserv_charge}\includegraphics[trim=2cm 9cm 1cm 9cm,  clip, width=0.23\textwidth,clip]{../figures/tenSave_impact_reserv_charge2}}
\squeezeup
	\caption{Impact of reservation charge.}\label{fig:impact_reserv_charge}
\end{figure}
\textbf{Impact of reservation charge.} In Fig.~\ref{fig:impact_reserv_charge},
we vary the reservation charge for \capname capacity under a fixed usage
charge of 20\textcent/kWh. We see that
the operator can increase its profit by over 35\%, while tenants
can save their costs by nearly 15\%.
Naturally, with an increase in the reservation charge, the operator's revenue increases
while tenants' cost reduction decreases.
In general, as tenants more aggressively
oversubscribe their contract capacity (i.e.,
emergency probability increases), \capname capacity is
more efficiently utilized, thus better benefiting
the operator and tenants. One exception is
that the operator loses more profit
if it does not charge reservation price
(unless it charges a really high usage price).
This is because to accommodate tenants'
 sprinting, the operator needs
to provision more capacity for maintaining
the same PDU-level emergency probability,
requiring more revenue
 to cover the
added infrastructure cost (for which
20\textcent/kWh usage charge with zero
reservation charge is not enough).






\begin{figure}[!t]
	\centering
	\subfigure[]{\label{fig:opSave_impact_usage_charge}\includegraphics[trim=2cm 9cm 1cm 9cm,  clip, width=0.23\textwidth,clip]{../figures/opSave_impact_usage_charge2}}
	\subfigure[]{\label{fig:tenSave_impact_usage_charge}\includegraphics[trim=2cm 9cm 1cm 9cm,  clip, width=0.23\textwidth,clip]{../figures/tenSave_impact_usage_charge2}}
\squeezeup
	\caption{Impact of usage charge.}\label{fig:impact_usage_charge}
\end{figure}

\textbf{Impact of usage charge.}
We now show the impact of usage charge in Fig.~\ref{fig:impact_usage_charge} with
a fixed 30\$/KW reservation charge for \capname capacity. Similar to the impact of reservation charge, the operator's profit increases with while
 tenants' cost saving reduces with the usage charge. Further, we
 see that operator can  even lose profit, if it
 does not charge
 tenants based on actual usage of \capname capacity
 while  tenants
 aggressively oversubscribe their capacity (with an emergency
 probability of 15\%).

 Combining
Fig.~\ref{fig:impact_reserv_charge} with Fig.~\ref{fig:impact_usage_charge},
we see that
there is a large range of reasonable
reservation and usage charges that can benefit
both the operator and tenants. This is because
tenants do not always have peak loads and their
aggregate peak is even rarer.
Thus, to keep the same PDU-level emergency probability
and
satisfy the operator's risk control policy,
the extra capacity provisioning
needed by the operator to accommodate tenants' increased
demand for occasional
capacity sprinting is really marginal. In other words,
capacity sprinting can be provisioned by the operator
almost for ``free'' with little extra cost (e.g.,
our result shows that when tenants each oversubscribe
the contract capacity by 20\% and have a 10\%
emergency, the operator only needs
to provision 3\% more PDU-level capacity to accommodate
tenants' sprinting).




\subsubsection{Performance Improvement}






To illustrate the performance improvement brought
by \ouralg, our power trace data is not applicable and we need
to run actual experiments. For this purpose, we
consider two representative tenants, one running
delay-sensitive key-value-store workloads (for
a multi-tier web service)
and the other running  Hadoop batch workloads (for data analytics).
They have 15\% and 25\% oversubscription over their contract capacity, respectively.
Fig.~\ref{fig:trace_tenants} shows the power and performance traces for a 10-minute experiment.
We see that with \ouralg, tenants can perform  sprinting by using more
power beyond their contract capacity and
avoid performance losses. Nonetheless,
without \ouralg, tenants
need to cap their power (using DVFS in our experiment)
and experience performance degradation: the 95-percentile delay for key-value-store
workloads can increase to over 700ms from 250ms, while the throughput
for Hadoop workloads may decrease by more than 50\% from 17kB/s to 8kB/s.

Thus, compared to leasing
additional capacity at full prices,
\ouralg provides a \emph{low-cost} solution to accommodate tenants' sprinting and
avoid performance degradation incurred by power capping techniques (e.g.,
power reduction or workload migration \cite{Wang:2013:VPD:2485922.2485973}).









\subsubsection{Sensitivity Study}


\begin{figure}[]
	\centering
	\subfigure[]{\label{fig:opSave_default}\includegraphics[trim=2cm 9cm 1cm 9cm,  clip, width=0.23\textwidth,clip]{../figures/opSave_default2}}
\subfigure[]{\label{fig:opSave_oversubscription_level}\includegraphics[trim=2cm 9cm 1cm 9cm,  clip, width=0.23\textwidth,clip]{../figures/opSave_impact_opOverSub}}
\squeezeup
	\caption{Sensitivity study. (a) Number of participating
tenants; (b) Operator's oversubscription levels.}\label{fig:err}
\end{figure}

\textbf{Number of participating tenants.} We now vary
the number of tenants participating  in \ouralg and show
the operator's profit increase in Fig.~\ref{fig:opSave_default}.
It can be seen that
 the operator's profit increases with tenants' oversubscription level as well as with
 the number of participating tenants. This is because different tenants
 typically utilize \capname capacity at different
 times and hence, with more participating tenants,
 the operator can better exploit multiplexing effects among
 tenants' power demand (i.e., sell more \capname capacity
 with little extra provisioning of the actual power/cooling capacity
 at the shared upper level). Individual tenant's cost
 saving remains the same regardless of the number of participating
 tenants, because \ouralg does not
 impose restrictions on when tenants can
 utilize \capname capacity as long as they have enough tokens.




\textbf{Operator's oversubscription levels.} The operator
can also take some risks and oversubscribe its own infrastructure capacity
by selling it to more tenants than the capacity allows \cite{Shaolei_Colocation_Power_Capping_HPCA_2016}.
We vary the operator's oversubscription levels, measured in the capacity emergency/overloading probability,
and show in Fig.~\ref{fig:opSave_oversubscription_level}
that by doing so, the operator can increase the average capacity utilization
and increase profit. Nonetheless,
\ouralg is not intended to help the operator with its oversubscription
(which was addressed by \cite{Shaolei_Colocation_Power_Capping_HPCA_2016});
instead, given any oversubscription level, \ouralg exploits the unused shared capacity
and utilizes it to accommodate tenants'  sprinting.
Thus, as shown in Fig.~\ref{fig:opSave_oversubscription_level}, \ouralg is complementary to the operator's oversubscription
strategy and can further increase its profit.








